Evaluating RAG-Fusion with RAGElo: an Automated Elo-based Framework

Challenges in the automated evaluation of Retrieval-Augmented Generation (RAG) Question-Answering (QA) systems include hallucination problems in domain-specific knowledge and the lack of gold standard benchmarks for company internal tasks. This results in difficulties in evaluating RAG variations, like RAG-Fusion (RAGF), in the context of a product QA task at Infineon Technologies. To solve these problems, we propose a comprehensive evaluation framework, which leverages Large Language Models (LLMs) to generate large datasets of synthetic queries based on real user queries and in-domain documents, uses LLM-as-a-judge to rate retrieved documents and answers, evaluates the quality of answers, and ranks different variants of Retrieval-Augmented Generation (RAG) agents with RAGElo's automated Elo-based competition. LLM-as-a-judge rating of a random sample of synthetic queries shows a moderate, positive correlation with domain expert scoring in relevance, accuracy, completeness, and precision. While RAGF outperformed RAG in Elo score, a significance analysis against expert annotations also shows that RAGF significantly outperforms RAG in completeness, but underperforms in precision. In addition, Infineon's RAGF assistant demonstrated slightly higher performance in document relevance based on MRR@5 scores. We find that RAGElo positively aligns with the preferences of human annotators, though due caution is still required. Finally, RAGF's approach leads to more complete answers based on expert annotations and better answers overall based on RAGElo's evaluation criteria.

==> sections/embeddings.tex <==
\section{Selection of Embedding Model}
Understanding the embedding model used in RAG-based systems is important to evaluate the quality of retrieved documents and the speed at which the documents are encoded and retrieved. If the retrieved documents are not relevant to the query, the chatbot is unable to provide a proper answer. In addition, slow encoding speed leads to both user frustration and server-based timeouts. This trade-off between accuracy and speed is a subject of research in itself \cite{rygl2017semantic}.

The Infineon RAG-Fusion and naive RAG systems both used the same Sentence Transformers embedding model, \textit{all-MiniLM-L6-v2}. The decision to use this model was reached by comparing the quality and speed of three Sentence Transformers \textit{all-*} embedding models: \textit{all-mpnet-base-v2}, and \textit{paraphrase-MiniLM-L3-v2}. These models were chosen because they respectively represent two extremes and one middleground of the accuracy and speed trade-off.

Mapping data tokens to vectors in a condensed space where similar tokens are closely positioned, embeddings are an essential part of RAG-based models \cite{azar2023estimation}. Sentence transformers, or Sentence-BERT, is an adaptation of the pre-trained BERT model enhanced with siamese and triplet network architectures for generating semantically significant sentence embeddings, enabling comparison through cosine-similarity, dot product, and euclidean distance measures \cite{reimers2019sentencebert}. \textit{All-*} Sentence Transformers models are trained on over one billion training pairs \cite{SBERTNET}. \textit{all-MiniLM-L6-v2} is a finetuned on 1 billion sentence pairs from a 6 layer version of Microsoft's distilled MiniLM model, \textit{MiniLM-L12-H384-uncased.} These models are also referred to as sentence or paragraph encoders \cite{chen2023subsentence}. MiniLM models have been evaluated for question generation and abstractive summarization, both tasks being key steps in the RAG-Fusion algorithm \cite{wang2020minilm}. Due to the large amount of training pairs and their focus for quality representations of not only sentences, but also search queries and paragraphs, they can be applied to RAG, which receives search queries from users and retrieves sentences and paragraphs from relevant documents. 

Key metrics for \textit{all-*} model evaluation include performance on sentence encoding, performance on semantic search, average performance over the two aforementioned scores, speed for encoding in sentences per second on a V100 GPU, and the size of the model in megabytes (MB). Based on the results provide by SBERT, the below table represents this evaluation for the three \textit{all-*} models we attempted to implement \cite{SBERTNET}.

\input{tables/embeddings}

The \textit{all-mpnet-base-v2} model offered the highest performance on semantic search and sentence embeddings; however, given the extremely low encoding speed, the chatbot was not able to produce answers within a reasonable amount of time. While the speed of the \textit{paraphrase-MiniLM-L3-v2} was significantly faster, performing embeddings and semantic search in a very short amount of time, the quality of answers significantly declined compared to \textit{all-mpnet-base-v2}.

\textit{all-MiniLM-L6-v2} transforms textual content, ranging from sentences to full paragraphs, into dense vectors of 384 dimensions. This functionality is particularly useful for semantic search and clustering tasks \cite{all-mini}. Since semantic search is used in the retrieval step of the RAG-Fusion algorithm, this model is applicable to RAG-Fusion \cite{RAGIFX}. Since \textit{all-MiniLM-L6-v2} provides a satisfactory middleground between the two, we implemented this model in our RAG and RAG-Fusion systems.

This model uses dot-product, cosine-similarity, and euclidean distance as suitable score functions to evaluate the similarity between distinct pieces of text \cite{suresh2024ragbased}. In this study, we use cosine similarity as a metric to represent semantic vector distance. The SentenceTransformers cosine similarity function outputs a matrix of cosine similarities based on two sets of embeddings \cite{SBERTNET}.

Given matrices \( \mathbf{A} = [\mathbf{a}_1, \mathbf{a}_2, \dots, \mathbf{a}_m] \) and \( \mathbf{B} = [\mathbf{b}_1, \mathbf{b}_2, \dots, \mathbf{b}_n] \), where each row \( \mathbf{a}_i \) and \( \mathbf{b}_j \) represents a vector, the cosine similarities between all pairs of vectors from \( \mathbf{A} \) and \( \mathbf{B} \) are calculated.
\[
\mathbf{C} = [c_{ij}] \quad \text{where} \quad c_{ij} = \frac{\mathbf{a}_i \cdot \mathbf{b}_j}{\|\mathbf{a}_i\| \|\mathbf{b}_j\|}
\]
\( \mathbf{C} \) is the resulting matrix of cosine similarities, and \( c_{ij} \) denotes the cosine similarity between vectors \( \mathbf{a}_i \) and \( \mathbf{b}_j \).

==> tables/embeddings.tex <==
\begin{table*}[ht]
\centering
 \caption{Comparison of Key Metrics from All-\* Embedding Models}\label{tab:embedding_comparison}
  \begin{tblr}{
    width=\textwidth,
    colspec={X[2,l] X[1,c] X[1,c] X[1,c] X[1,c] X[1,c] X[1,c]},
    colsep=1pt,
    rowsep=0pt,
    row{odd}={bg=azure9},
    row{1} = {c, bg=azure3, fg=white, cmd=\bfseries}
  }
    Model Name & Sentence Embeddings & Semantic Search & Average & Speed  & Model Size \\
    all-mpnet-base-v2       & 69.57 & 57.02 & 63.30 & 2800  & 420 MB \\
    all-MiniLM-L6-v2        & 68.06 & 49.54 & 58.80 & 14200 & 80 MB  \\
    paraphrase-MiniLM-L3-v2 & 62.29 & 39.19 & 50.74 & 19000 & 61 MB  \\
  \end{tblr}%
\end{table*}

==> tables/scores.tex <==
\begin{table*}[ht]
\centering
 \caption{Summary of Human and LLM Annotations}\label{tab:llm_annotations}
  \begin{tblr}{
    width=\columnwidth,
    colspec={X[l, -1]},
    colsep=1pt,
    rowsep=0pt,
    row{odd}={bg=azure9},
    column{1} = {cmd=\small},
    row{1} = {c, bg=azure3, fg=white, font=\sffamily, cmd=\textbf},
    hline{1,Z} = {solid, 1pt},
  }
    Agent & Rater & Category & Number of 2's & Number of 1's & Number of 0's & Mean \\
    RAG   & LLM     & Relevance     & 18 & 1 & 1  & 1.85  \\
    RAG   & Human   & Relevance     & 16 & 4 & 0  & 1.80  \\
    RAG   & LLM     & Accuracy      & 16 & 3 & 1  & 1.75  \\
    RAG   & Human   & Accuracy      & 17 & 2 & 1  & 1.80  \\
    RAG   & LLM     & Completeness  & 14 & 5 & 1  & 1.65  \\
    RAG   & Human   & Completeness  & 10 & 7 & 3  & 1.65  \\

  \end{tblr}%
\end{table*}
